Direction-Constrained Control for Efficient Physical Human-Robot Interaction under Hierarchical Tasks

This paper proposes a control method to address the physical Human-Robot Interaction (pHRI) challenge in the context of hierarchical tasks. A common approach to managing hierarchical tasks is Hierarchical Quadratic Programming (HQP), which, however, cannot be directly applied to human interaction due to its allowance of arbitrary velocity direction adjustments. To resolve this limitation, we introduce the concept of directional constraints and develop a direction-constrained optimization algorithm to handle the nonlinearities induced by these constraints. The algorithm solves two sub-problems, minimizing the error and minimizing the deviation angle, in parallel, and combines the results of the two sub-problems to produce a final optimal outcome. The mutual influence between these two sub-problems is analyzed to determine the best parameter for combination. Additionally, the velocity objective in our control framework is computed using a variable admittance controller. Traditional admittance control does not account for constraints. To address this issue, we propose a variable admittance control method to adjust control objectives dynamically. The method helps reduce the deviation between robot velocity and human intention at the constraint boundaries, thereby enhancing interaction efficiency. We evaluate the proposed method in scenarios where a human operator physically interacts with a 7-degree-of-freedom robotic arm. The results highlight the importance of incorporating directional constraints in pHRI for hierarchical tasks. Compared to existing methods, our approach generates smoother robotic trajectories during interaction while avoiding interaction delays at the constraint boundaries.

==> tex/9Biography.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/Author_Mengxin Xu.pdf}}]
{Mengxin Xu}
received the B.S. degree in automation science in 2020, from Shanghai Jiao Tong University, Shanghai, China, where he is currently working toward the Ph.D. degree in control science and engineering.

His current research interests include vision-based aerial manipulation, impedance control of aerial robots and aerial vehicle design.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/Author_Hesheng Wang.pdf}}]
{Hesheng Wang}
(SM’15) received the
B.Eng. degree in electrical engineering
from the Harbin Institute of Technology,
Harbin, China, in 2002, and the M.Phil.
and Ph.D. degrees in automation and
computer-aided engineering from The
Chinese University of Hong Kong, Hong
Kong, in 2004 and 2007, respectively.
He was a Postdoctoral Fellow and
Research Assistant with the Department of Mechanical and
Automation Engineering, The Chinese University of Hong
Kong, from 2007 to 2009. He is currently a Professor with the
Department of Automation, Shanghai Jiao Tong University,
Shanghai, China. His current research interests include visual
servoing, service robot, and autonomous driving.

Dr. Wang is an Associate Editor of \emph{Assembly Automation and
the International Journal of Humanoid Robotics}, a Technical
Editor of the IEEE/ASME \textsc{Transactions on Mechatronics}.
He served as an Associate Editor of the IEEE
\textsc{Transactions on Robotics} from 2015 to 2019. He was the
General Chair of the IEEE \textsc{Real-time Computing and Robotics}
(RCAR) in 2016, and the Program Chair of the IEEE \textsc{Robotics
and Biomimetics} (ROBIO) in 2014 and IEEE/ASME \textsc{Advanced
Intelligent Mechatronics} (AIM) in 2019.

\end{IEEEbiography}
